Artificial Neural Network for Resource Allocation in Laser-based Optical wireless Networks

Optical wireless communication offers unprecedented communication speeds that can support the massive use of the Internet on a daily basis. In indoor environments, optical wireless networks are usually multi-user multiple-input multiple-output (MU-MIMO) systems, where a high number of optical access points (APs) is required to ensure coverage. In this work, a laser-based optical wireless network is considered for serving multiple users. Moreover, blind inference alignment (BIA) is implemented to achieve a high degree of freedom (DoF) without the need for channel state information (CSI) at transmitters, which is difficult to provide in such wireless networks. Then, an objective function is defined to allocate the resources of the network taking into consideration the requirements of users and the available resources. This optimization problem can be solved through exhaustive search or distributed algorithms. However, a practical algorithm that provides immediate solutions in real time scenarios is required. In this context, an artificial neural network (ANN) model is derived in order to obtain a sub-optimal solution with low computational time. The implementation of the ANN model involves three important steps, dataset generation, offline training, and real time application. The results show that the trained ANN model provides a significant solution close to the optimal one.

==> main.tex <==

\input{./conference_101719.tex} %Preamble
\begin{document}
\frontmatter
\input{./IEEEtran.cls}
\input{./figures/fig.pdf}
\maketitle
\tableofcontents{}
\mainmatter
    %...\input various %
    %...\chapters ...  %     
\end{document}


==> source files (2)/main.tex <==

\input{./conference_101719.tex} %Preamble
\begin{document}
\frontmatter
\input{./IEEEtran.cls}
\input{./figures/fig.pdf}
\maketitle
\tableofcontents{}
\mainmatter
    %...\input various %
    %...\chapters ...  %     
\end{document}

